Convex-Concave Min-Max Stackelberg Games

Min-max optimization problems (i.e., min-max games) have been attracting a great deal of attention because of their applicability to a wide range of machine learning problems. Although significant progress has been made recently, the literature to date has focused on games with independent strategy sets; little is known about solving games with dependent strategy sets, which can be characterized as min-max Stackelberg games. We introduce two first-order methods that solve a large class of convex-concave min-max Stackelberg games, and show that our methods converge in polynomial time. Min-max Stackelberg games were first studied by Wald, under the posthumous name of Wald's maximin model, a variant of which is the main paradigm used in robust optimization, which means that our methods can likewise solve many convex robust optimization problems. We observe that the computation of competitive equilibria in Fisher markets also comprises a min-max Stackelberg game. Further, we demonstrate the efficacy and efficiency of our algorithms in practice by computing competitive equilibria in Fisher markets with varying utility structures. Our experiments suggest potential ways to extend our theoretical results, by demonstrating how different smoothness properties can affect the convergence rate of our algorithms.

==> ALGO_new_version <==
Restate the marginal function as a Lagrangian.
was max_{y in constraint set} f(x, y)
now max_{y, \lambda} f(x, y) - \lambda (constraints)

Outer loop intution: descend (one step) along the gradient of the marginal function wrt \outer
-- in practice, compute the gradient of the aformentioned Lagrangian wrt \outer, given \innerpoint and \langmultpoint

Inner loop intuition: ascend (til convergence; hence nested!) along the gradient of the objective function wrt \inner
-- in practice, run simultaneous GDA to solve for the optimal \inner and \langmult, given \outerpoint

N.B. in Fisher markets, we can solve for the optimal Lagrange multipliers in closed form, so it is not necessary to run the inner loop til convergence. the game thus becomes a Nash game instead of a Stackelberg game, which can be solved via simGDA.
\amy{???}
\amy{is this true in general? when you can solve for the Lagrange multipliers in closed form, say in convex-concave games, then does nested GDA reduce to sim GDA?}


==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%

\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Discussion in conclusion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Broader impacts section included.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Main assumption is given in \cref{main-assum} and other auxiliary assumptions are given in theorem statements}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Yes, all results' proofs can be found in the appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Information for replication are found on \cref{sec-app:fisher}. Instructions to run our code can be found on the readme.md of \coderepo}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details can be found in \cref{sec-app:fisher}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details can be found in \cref{sec-app:fisher}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Can be found in \cref{sec-app:fisher}}
  \item Did you mention the license of the assets?
    \answerYes{Can be found in \cref{sec-app:fisher}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Code and assets can be found on \coderepo.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> continuous.tex <==

\section{Min-Max Optimization with Variable Choice Set Beyond Convex-Concave Settings}

We will now consider a continuous time variant of the max-oracle algorithm \ref{mogd}, to extend convergence results of the algorithm to a class of non-convex-concave settings. Unfortunately, the translation of the algorithm into a continuous time dynamical system is not straightforward since in the discrete time algorithm each calculated iterate is projected back onto the set feasible set $\outers$. For simplicity, we will define a continuous time process assuming $\outers = \R^\outerdim$, however, note that our results can be generalized for any compact convex $\outers$ by assuming that the flow we define is on a Riemannian manifold defineing the set $\outers$. Before moving forward, we define some important concepts. This simplification does not change the structure of the problem significantly since the difficulty of solving min-max optimization problems with variable choice sets stems from the constraints of the $\inner$-player being dependent of the action of the $\outer$-player, a structure which our assumption does not affect. A flow is a function $\flow:  \R \times \R^{\outerdim}  \to \R^\outerdim$, $(t, \outer) \to \flow[t](\outer)$ that describes the value of a variable that has initial value $\outer \in \R^\outerdim$ at some time $t$. A gradient flow is an flow such that:

\begin{align}
    \frac{\partial}{\partial t} \flow[t](\outer) = - \grad[\outer] \val(\outer)
\end{align}
La Salle's Invariance principle \cite{lasalle1960grad} gives the sufficient condition under which this flow asymptotically converges to a stationary point.

\begin{theorem}[La Salle Invariance Principle \cite{lasalle1960grad}]
    Let $\val: \R^\outerdim \to \R$ be a continuously differentiable function a.e. with compact sublevel sets, i.e., $K_\alpha = \left\{ \outer \in \outers \mid  \val(\outer) \leq \alpha \right\}$. is compact for all $\alpha \in (-\infty, \infty)$, then for any $\outer \in \outers$, $\lim_{t \to \infty} \flow[t](\outer)$ exists and converges to an element of the set $\left\{\z \mid \grad[\outer]\val(\z) = 0 \right\}$.
\end{theorem}

We can define a continuous time-version of algorithm \ref{mogd} as a dynamical system with phase space $\outers$ and evolution function given by:

\begin{align}\label{continuous-time}
    \frac{\partial}{\partial t} \flow[t](\outer) = \grad[\outer] \obj(\outer, \inner^*(\outer)) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr](\outer) \grad[\outer]  \constr[\numconstr](\outer, \inner^*(\outer))
\end{align}
where $\langmult(\outer)$ are the Lagrange multipliers associated with $\inner^*(\outer)$.

By \Cref{envelope}, we know that $\grad \val(\outer) = \grad[\outer] \obj(\outer, \inner^*(\outer)) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr](\outer) \grad[\outer]  \constr[\numconstr](\outer, \inner^*(\outer))$, where $\val(\outer) = \val(\outer) = \max_{\inner : g(\outer, \inner) \geq 0} \obj(\outer, \inner)$. Hence, \Cref{continuous-time} is the gradient flow defined by the value function $\val(\outer)$. Unfortunately, La Salle's invariance principle cannot be applied to show that \Cref{continuous-time} asymptotically converges to a stationary point of $\val$, since by \Cref{no-danskins-ex}, \Cref{value-func-deriv-example}, we know that for even very simple maximization problem with variable choice sets, the value function is not differentiable. However, \Cref{envelope} guarantees that the value function $\val$ is absolutely continuous which means that it is differentiable almost everywhere. This property can allow us to reach the conclusions of La Salle's invariance principle for without assuming that the value function is continuously differentiable. We formalize this inutition in \Cref{our-very-own-lasalle}:

\begin{theorem}\label{our-very-own-lasalle}
    Let $f$ be a continuous function $f: \R^{\outerdim} \times \R^{\innerdim} \to \mathbb{R}$ that is concave in $\inner$ with partial derivative with respect to $\outer$ continuous in $\outer$ and $\inner$, and  which has compact sublevel set with respect to $\outer$, i.e., $\left\{ \outer \in \outers \mid \obj(\outer, \inner) \leq \alpha  \text{ for all } \inner \in \inners(\outer)\right\}$ is compact for all $\alpha \in (-\infty, \infty)$. Additionally, assume that there is some $\widehat{\inner} \in \mathbb{R}^{n}$
    such that $g_{k}(\outer, \widehat{\inner})>0$ for all $k=1, \ldots, K$ and all $\outer \in \R^m$, that the sublevel set of $\obj$ are compact for all $\inner$ and $\obj$ is Lipschitz in f. Consider the flow defined in \Cref{continuous-time}, then for any $\outer \in \outers$, $\lim_{t \to \infty} \flow[t](\outer)$ exists and converges to an element of the set $\left\{\z \mid \grad[\outer]\val(\z) = 0 \right\}$.
\end{theorem}

\begin{proof}
First, note that by \Cref{envelope} $\grad \val(\outer) = \grad[\outer] \obj(\outer, \inner^*(\outer)) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr](\outer) \grad[\outer]  \constr[\numconstr](\outer, \inner^*(\outer))$, and that $\val$ is almost absolutely continuous, where $\val(\outer) = \val(\outer) = \max_{\inner : g(\outer, \inner) \geq 0} \obj(\outer, \inner)$.  Let $v(t) = \val(\potential[t](\outer))$ denote the value along the curve defined by $\potential[t](\outer)$ with starting point $\outer$. We then have:
\begin{align}
    \frac{dv}{dt} &= \grad \val(\potential[t](\outer)) \cdot \frac{d\potential[t]}{dt}\\
    &= \grad \val(\potential[t](\outer)) \cdot \left(\grad[\outer] \obj(\potential[t](\outer), \inner^*(\potential[t](\outer))) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr](\potential[t](\outer)) \grad[\outer]  \constr[\numconstr](\potential[t](\outer), \inner^*(\potential[t](\outer)))\right) && \text{(\Cref{continuous-time})}\\
    &= \grad \val(\potential[t](\outer)) \cdot (- \grad \val(\potential[t](\outer)) ) && \text{(\Cref{envelope-deriv})}\\
    &= - \left\|\grad \val(\potential[t](\outer)) )\right\|^2 
\end{align}
Since $\val$ is absolutely continuous, it is differentiable almost everywhere and $\grad \val(\potential[t](\outer))$ is Lebesgue integrable. Hence, the following integral equation is well defined:
\begin{align}
    v(t) = v(0) + \int_0^t - \left\|\grad \val(\potential[t](\outer)) )\right\|^2\\
    v(t) = v(0) - \int_0^t\left\|\grad \val(\potential[t](\outer)) )\right\|^2
\end{align}
\end{proof}

\begin{lemma}
Let $f$ be a continuous function $f: \R^{\outerdim} \times \R^{\innerdim} \to \mathbb{R}$ which has compact sublevel set with respect to $\outer$, i.e., $\left\{ \outer \in \outers \mid \obj(\outer, \inner) \leq \alpha  \text{ for all } \inner \in \inners(\outer)\right\}$ is compact for all $\alpha \in (-\infty, \infty)$, then $\left\{ \outer \in \outers \mid \val(\outer) \leq \alpha \right\}$ is compact as well.
\end{lemma}

==> discussion.tex <==
\section{Discussion}
\deni{Remove this section}
% \amy{cut from elsewhere}
\sdeni{The intuition behind algorithm \ref{mogd}, is to essentially run (sub)gradient descent on the value function since by \Cref{envelope-sd}, we have a formula for the subdifferential set of the value function. Note that as opposed to the fixed choice set setting, even very simple value functions are not differentiable. However, by \Cref{envelope}, the inner value function is absolutely continuous meaning that it is differentiable almost everywhere, and, as a result, the probability that the algorithm will encounter a non-differentiable point is low if not zero. That said, \Cref{envelope-sd}, guarantees that the step calculated at each step will also be a subgradient at non-differentiable points of the value function. That said, since the inner value function is not differentiable in general it is unlikely that there exists a first-order method that converges in last iterate to the Stackelberg equilibrium of a min-max game with variable choice sets, even with a convex-concave objective functions. The intuition behind this is similar to the non-convergence of subgradient methods in last iterates.}{}

A worthwhile question to explore would be to derive stronger conditions under which the inner value function $\val$ Lipschitz-smooth to achieve better convergence results under stronger assumptions. In order for $\val$ to be differentiable, the subdifferential of value function given by \Cref{envelope-sd} needs to be a singleton for all $\outer \in \outerset$. This means that not only the solution function $\innerset^{*}(\outer)$ has to be a singelton for all $\outer \in \outers$ but the optimal Lagrangian multipliers function $ \langmults(\widehat{\outer}, \inner^{*}(\widehat{\outer})))$ have to also be singleton-valued. The former can be guaranteed when $\obj$ is strictly concave in $\inner$, while the later condition is satisfied when the Linear Independence Constraint Qualification (LICQ) condition \cite{henrion1992constraint} holds. However, even when both conditions hold, the conditions required on the objective function and choice set of the inner player for the gradient of the value function to be Lipschitz-smooth are not clear. In particular, even if the objective function and the functions defining the constraints of the inner player are Lipschitz-smooth, it is not clear how one would derive conditions for the product of the Langrange multipliers (which are a function of the outer player's action) with the gradient of the functions defining the dependency constraints to be Lipschitz-smooth. 

Additionally, it is not straightforward what conditions should be used to extend convergence results to non-convex-non-concave domains, as previously used conditions seem to not apply to the dependent strategy sets regime. For instance, \citeauthor{nouiehed2019solving} exploit the fact that when the objective function satisfies the Lojasiewicz condition, the value function also satisfies it to prove that their multistep algorithm can solve a class of non-convex min-max games \cite{nouiehed2019solving}. However, since the gradient of the value function of min-max games with dependent strategy sets are also a function of the constraints, and optimal Langragian multipliers of the problem, the same intuition no more applies. Additionally, \citeauthor{nouiehed2019solving} show that when the objective function satisfies the Lojasiewicz condition the value function of the problem also becomes differentiable, a result that does not transfer to the value functions of min-max games with dependent strategy sets.
\deni{Should anything be cut in the next two paragraphs? Seems too long.}



==> fisherproofs.tex <==
\subsection{Omitted Proofs \Cref{sec:fisher}}

\begin{proof}[Proof of optimality of \Cref{fisher-obj}]
Firstly, note that since $\util[\buyer]$ is assumed to be concave for all $\buyer \in \buyers$, we know that the objective function is concave in $\allocation$. Additionally, since the only term in \Cref{fisher-obj} dealing with $\price$ is affine, the objective function is convex in $\price$. Hence, \Cref{fisher-obj} is a convex-concave min-max optimization problem with dependent strategy sets. The value function of the inner optimization problem in \Cref{fisher-obj} is given by:
\begin{align}
    \val(\price) = \max_{\allocation: \allocation \price \leq \budget} \sum_{\good \in \goods} \price[\good] +  \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer])\right)
\end{align}
%
Let $\langmult \in \R^\numbuyers$ and $\bm \mu \in \R^{\numbuyers \times \numgoods}$ be the Lagrange multipliers associated with the budget and non-negativity constraints respectively. The Lagrangian associated with the above optimization problem is given by:
\begin{align}
    L(\allocation, \langmult, \bm{\mu}) = \sum_{\good \in \goods} \price[\good] +  \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer])\right) + \sum_{\buyer \in \buyers} \langmult[\buyer] \left(\budget[\buyer]  - \allocation[\buyer] \cdot \price \right) - \sum_{\substack{\buyer \in \buyers\\ \good \in \goods}} \mu_{\buyer \good} \allocation[\buyer][\good]
\end{align}

The optimal variables $(\allocation^*, \langmult^*, \bm{\mu}^*)$ for the Lagrangian above satisfy the KKT slack complementarity condition \cite{kuhn1951kkt}:
%
\begin{align}
    \langmult[\buyer]^*(\budget[\buyer] -\allocation[\buyer]^* \cdot \price ) = 0 && \forall \buyer \in \buyers\\
    \langmult[\buyer]^* > 0 \implies \allocation[\buyer]^* \cdot \price  = \budget[\buyer]\label{budget-constr}
\end{align}
\amy{budget constraint is respected}
and 
\begin{align}
    \mu_{\buyer \good}^* \allocation[\buyer][\good]^* = 0\label{non-neg-kkt}
\end{align}
%
as well as the KKT stationarity condition:
\amy{which implies $\lambda$'s optimal value}
\begin{align}
    - \frac{\budget[\buyer]}{\util[\buyer](\allocation[\buyer]^*)} \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer] = \allocation[\buyer]^*} + \langmult[\buyer]^* \price[\good] - \mu_{ij}^* = 0 && \forall \buyer \in \buyers, \good \in \goods\\
    \langmult[\buyer]^* \price[\good] \allocation[\buyer][\good]^* - \mu_{ij}^*\allocation[\buyer][\good]^* =  \frac{\budget[\buyer]}{\util[\buyer](\allocation[\buyer]^*)} \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer]  = \allocation[\buyer]^*} \allocation[\buyer][\good]^* && \forall \buyer \in \buyers, \good \in \goods
\end{align}
where the last line was obtained by multiplying both sides by $\allocation[\buyer][\good]^*$ and re-organizing expressions. By \Cref{non-neg-kkt}, we have $\mu_{ij}^*\allocation[\buyer][\good]^* = 0$, giving us:
\begin{align}
    \langmult[\buyer]^* \price[\good] \allocation[\buyer][\good]^*  =  \frac{\budget[\buyer]}{\util[\buyer](\allocation[\buyer]^*)} \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer]  = \allocation[\buyer]^*} \allocation[\buyer][\good]^* && \forall \buyer \in \buyers, \good \in \goods
\end{align}
Summing up across $\good$'s we obtain:
\begin{align}
    \langmult[\buyer]^* \sum_{\good \in \goods} \price[\good] \allocation[\buyer][\good]^*  =   \frac{\budget[\buyer]}{\util[\buyer](\allocation[\buyer]^*)} \sum_{\good \in \goods} \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer]  = \allocation[\buyer]^*} \allocation[\buyer][\good]^* && \forall \buyer \in \buyers, \good \in \goods\\
    \langmult[\buyer]^* \sum_{\good \in \goods} \price[\good] \allocation[\buyer][\good]^*  =   \frac{\budget[\buyer]}{\util[\buyer](\allocation[\buyer]^*)}\label{eq:homo-euler} \util[\buyer](\allocation[\buyer]^*) && \forall \buyer \in \buyers, \good \in \goods\\
    \langmult[\buyer]^* \sum_{\good \in \goods} \price[\good] \allocation[\buyer][\good]^*  =   \budget[\buyer] && \forall \buyer \in \buyers, \good \in \goods
\end{align}
where the penultimate line was obtained from Euler's theorem for homogeneous functions \cite{border2017euler}. Finally, since $\budget[\buyer] > 0$ by the assumptions of the model, both $ \langmult[\buyer]^*$ and $\left( \allocation[\buyer]^* \cdot \price\right)$ have to be positive for the equality to hold. Hence, we can substitute in \Cref{budget-constr} and obtain:
\begin{align}
    \langmult[\buyer]^* \left( \allocation[\buyer]^* \cdot \price\right) =   \budget[\buyer] && \forall \buyer \in \buyers, \good \in \goods\\
    \langmult[\buyer]^* \budget[\buyer]  =   \budget[\buyer] && \forall \buyer \in \buyers, \good \in \goods\\
    \langmult[\buyer]^*   =   1 && \forall \buyer \in \buyers, \good \in \goods\label{langmulteq1}
\end{align}
Hence, the Lagrange multiplier $\langmult[\buyer](\price, \allocation^*(\price))$ associated with $\allocation^*(\price)$ is unique and equal to 1. Additionally, note that we then have from the KKT stationarity:
\begin{align}
    \text{if } \allocation[\buyer][\good]^* > 0 \implies \langmult[\buyer]^* \frac{\util[\buyer](\allocation[\buyer]^*)}{\budget[\buyer]} = \frac{\left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer] = \allocation[\buyer]^*}}{\price[\good]} && \forall \buyer \in \buyers, \good \in \goods\\
    \text{if } \allocation[\buyer][\good]^* > 0 \implies  \frac{\util[\buyer](\allocation[\buyer]^*)}{\budget[\buyer]} = \frac{\left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer] = \allocation[\buyer]^*}}{\price[\good]}\label{equimarginal} && \forall \buyer \in \buyers, \good \in \goods
\end{align}
In other words, \Cref{equimarginal} states that $\allocation^*$ satisfies the optimality conditions for $\allocation^*$ to be utility maximizing at budgets $\budget$ \cite{market-notes}, while \Cref{budget-constr} confirms that buyers do not spend more than their budget. As a result, combining \Cref{budget-constr} and \Cref{equimarginal}, we can clearly see that the inner optimization problem in \Cref{fisher-obj} solves for utility maximizing allocations $\allocation^*$ constrained by the buyers' budgets.
\amy{equi-marginal principle; potential function models how far away economy is from equi-marginal principle}

We will now show that the optimal prices $\price$ which correspond to a Stackelberg equilibrium of \Cref{fisher-obj}, are market clearing and utility maximizing. By the envelope \Cref{envelope} the derivative of the value function at points it is differentiable is given by:
\amy{this envelope theorem only applies in the special case where the value function is differentiable}
\amy{the gradient of the value function (i.e., welfare = seller's prices (constant) plus total buyer's utilities) is the excess demand (n.b. excess demand is unique)}
%
\begin{align}
    \grad[\price] \val(\widehat{\price}) &= \grad[\price] \left[ \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer] (\allocation[\buyer](\widehat{\price}), \budget[\buyer])\right) \right] + \sum_{\buyer \in \buyers} \langmult[\buyer] \grad[\price] \left( \budget[\buyer] - \allocation[\buyer]^* (\widehat{\price}, \budget[\buyer]) \cdot \price  \right) \\
    &= \ones[\numgoods] - \sum_{\buyer \in \buyers} \langmult[\buyer] \allocation[\buyer]^* (\widehat{\price}, \budget[\buyer]) \\
    &= \ones[\numgoods] - \sum_{\buyer \in \buyers} \allocation[\buyer]^* (\widehat{\price}, \budget[\buyer]) && \text{(\Cref{langmulteq1})}
 \end{align}
 %
Let $\outerset^*(\price, \budget) = \argmax_{\allocation : \allocation \price \leq \budget} \util[\buyer](\allocation[\buyer])$. More generally, the subdifferential of the value function is given by \Cref{envelope-sd}:
%
\begin{align}
    \subdiff[\price] \val(\price) &= \mathrm{conv}\left( \bigcup_{\allocation[\buyer]^*(\price, \budget[\buyer]) \in \outerset^*(\price, \budget)} \left\{ \ones[\numgoods] - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price, \budget[\buyer]) \right\}\right) \\
    &=  \ones[\numgoods] - \mathrm{conv}\left( \bigcup_{\allocation[\buyer]^*(\price, \budget[\buyer]) \in \outerset^*(\price, \budget)} \left\{ \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price, \budget[\buyer]) \right\}\right) \\
    &=  \ones[\numgoods] -  \sum_{\buyer \in \buyers} \mathrm{conv}\left( \bigcup_{\allocation[\buyer]^*(\price, \budget[\buyer]) \in \outerset^*(\price, \budget)} \left\{ \allocation[\buyer]^*(\price, \budget[\buyer]) \right\}\right) \\
    &= \ones[\numgoods] -  \sum_{\buyer \in \buyers}  \outerset^*(\price, \budget)
\end{align}
where the sum of set valued quantities is defined as the Minkowski sum of sets and the last line follows from the convexity of $\outerset^*(\price, \budget)$. That is, the subdifferential of the value function is equal to the set of excess demands in the market.

The optimality condition for a price vector $\price^*$ to be a minimum of the outer minimization problem in \Cref{fisher-obj} is given as:
%
\begin{align}
    \{0\} \in \subdiff[\price] \val(\price^*) = \ones[\numgoods] -  \sum_{\buyer \in \buyers}  \outerset^*(\price^*, \budget)
\end{align}
The above condition simply states that at prices $\price^*$, there is a market clearing vector of demands that are utility maximizing constrained by budget. Letting $\allocation^*(\price^*) \in \outerset^*(\price^*, \budget)$, we have that any Stackelberg equilibrium $(\allocation^*(\price^*, \budget[\buyer]), \price^*)$ of \Cref{fisher-obj} is a competitive equilibrium.
\end{proof}


==> intro_from_stoch_paper.tex <==

\deni{All of this below will be removed and replaced with a thorough contributions and related works section.}
\sdeni{}{Nearly a century after von Neumann's initial inquiry into min-max optimization, resulting in his seminal minimax theorem \cite{neumann1928theorie}, min-max optimization has once again become an important research topic, due its machine learning applications, including but not limited to generative adversarial networks (GANs) \cite{goodfellow2014gan}, statistical learning \cite{xu2009robustness, shafieezadeh2015distributionally, dai2019kernel}, online learning \cite{cesa2006prediction}, deep learning \cite{sinha2017certifiable, sinha2020certifying}, distributed computing \cite{shamma2008cooperative, mateos2010distributed}, fairness in machine learning \cite{dai2019kernel, edwards2016censoring, madras2018learning, sattigeri2018fairness, xu2018fairgan}, and generative adversarial imitation learning \cite{cai2019global, hamedani2018iteration}.
These \amy{All? Some? Many?} applications require one to solve a \mydef{stochastic (uncoupled) constrained min-max optimization problem}, i.e., 
$$\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner) \doteq \Ex_{\obji \sim \objdistrib} \left[ \obj[\obji](\outer, \inner) \right] \enspace ,$$
% \deni{Should we change this to $\inf_{\outer \in \outerset} \sup_{\inner \in \innerset} \obj(\outer, \inner)$? Because, without the assumption that the sets are compact and the objective is continuous the min and max are not guaranteed to exist. I know that is straightforward but Costis seems to be careful with that in his paper, so maybe we should be too?} \amy{it's just a question of where we want to introduce these assumptions. we can do so right now, so that min and max are well-defined. is there any downside? we only really consider this case anyway, correct?}
where $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ are the constraint sets, $\objdistrib \in \simplex(\objs)$ is a probability distribution over a family of \mydef{\samy{objective}{} parameters} \amy{not sure? but seems wordy?} $\objs$, defining for each parameter $\obji \in \objs$, an \mydef{objective function} $\obj[\obji]: \R^\outerdim \times \R^\innerdim \to \R$. Here, it is assumed that for all parameters $\obji \in \objs$, the objective function $\obj[\obji]$ is continuous and the constraint sets $\outerset$ and $\innerset$ are non-empty and compact, assumptions which ensure that a solution to this optimization problem exists.

If in addition one assumes that the constraint sets $\outerset$ and $\innerset$ are convex, and that for each parameter $\obji \in \objs$, the objective function $\obj[\obji]$ is convex in $\outer$ for all $\inner \in \innerset$, and concave in $\inner$ for all $\outer \in \outerset$, i.e., $\obj[\obji]$ is \mydef{convex-concave}, then $\obj$ is convex-concave and in turn Sion's minimax theorem \cite{sion1958general}, a generalization of von Neumann's holds, guaranteeing the existence of a particular type of solution known as a \mydef{saddle point}, i.e., a point $(\outer[][][*], \inner[][][*]) \in \outerset \times \innerset$ s.t.\ for all $\outer \in \outerset$ and $\inner \in \innerset$, $\obj(\outer[][][*], \inner) \leq \obj(\outer[][][*], \inner[][][*]) \leq \obj(\outer, \inner[][][*])$.  

As a saddle point is simultaneously a minimum of $\obj$ in the $\outer$-direction and a maximum of $\obj$ in the $\inner$-direction, we can interpret such optimization problems as simultaneous-move zero-sum games \cite{neumann1928theorie, nash1950existence} \amy{don't have to cite Nash, i don't think, for the zero-sum case? unless i am missing something?} between an $\outer$- and $\inner$-player with respective action sets $\outerset$ and $\innerset$, and expected payoff functions $- \obj$, $\obj$, in which case $\outer[][][*]$ (resp.\ $\inner[][][*]$) can be interpreted as a best-response of the $\outer$- (resp.\ $\inner$-) player to their opponent's action $\inner[][][*]$ (resp.\ $\outer[][][*])$.
As such, \samy{the optimization problem can be interpreted as a (simultaneous-move) game,}
% \footnote{Throughout this paper, we refer to games with stochatic payoffs as stochastic games, and use the Markov game terminology to refer to repeated games with stochastic transitions first introduced by \citeauthor{shapley1953stochastic}  \cite{shapley1953stochastic}.}
{any saddle point of min-max optimization problem can be interpreted as a \mydef{Nash equilibrium of a zero-sum game} \cite{nash1950existence}.}
Note, however, that not all solutions to min-max optimization problems are saddle points and hence Nash equilibria. \amy{really? please explain!} \amy{maybe you are referring to the generalized case? but that is not the context right now.}

More generally, one might consider a \mydef{stochastic coupled constrained min-max optimization problem}, where the $\outer$ and $\inner$ variables are in addition required to lie within a \mydef{coupled constraints set} $\coupledset \subset \R^\outerdim \times \R^\innerdim$, \deni{Maybe making constraints parametrized is clearer?}
% constraints of the inner maximization problem depend on the selection for the maximization  problem via an \mydef{expected coupling constraint} $\constr(\outer, \inner) \doteq \Ex_{\constri \sim \constrdistrib} \left[\constr[\constri](\outer, \inner)\right]$ 
i.e.,
% $(\outerset, \innerset, \{\obj[\obji] \}_\obji, \{\constr[\constri] \}_\constri)$:
% \begin{align}\label{eq:stoch_minmax}
$$\min_{\outer \in \outerset} \max_{\inner \in \innerset: (\outer, \inner) \in \coupledset} \obj(\outer, \inner) \doteq \Ex_{\obji \sim \objdistrib} \left[ \obj[\obji](\outer, \inner) \right] \enspace , 
$$
% \end{align}
where the constraint sets $\outerset$ and $\innerset$, the objective parameter distribution $\objdistrib$, and the objective functions $\{\obj[\obji]\}_{\obji \in \objs}$ are defined as above.
Here, \amy{to guarantee existence once again? if so, say so!} it is assumed that the constraint sets $\outerset$, $\innerset$, and $\coupledset$ are non-empty and compact, with $\coupledset$ additionally strictly convex,%
\footnote{We note that the strict convexity assumption can be relaxed if one \samy{in addition}{instead} assumes that the interior of $\coupledset$ is non-empty.}
and for each parameters $\obji \in \objs$, the objective function $\obj[\obji]$ is continuous.
% , with the constraint functions additionally satisfying Slater's condition, i.e., $\forall \outer \in \outerset, \exists \inner \in \innerset$ s.t. $\constr[\constri](\outer, \inner) > 0$ for a solution to the optimization problem to exist

% constraint parameter distribution $\constrdistrib \in \simplex(\constrs)$ over a set of \mydef{constraint parameters} $\constrs$ that induce for each parameter $\constri \in \constrs$ a \mydef{coupling constraint} $\constr[\constri]: \R^\outerdim \times \R^\innerdim \to \R^\numconstrs$ on the optimization problem, which we require to be positive for any solution $(\outer[][][*], \inner[][][*])$, i.e., for all $\numconstr \in [\numconstrs]$, $\constr[\constri][\numconstr](\outer[][][*], \inner[][][*]) \geq 0$. Here, it is assumed that the constraint sets $\outerset, \innerset$ are non-empty and compact with $\innerset$ additionally convex, and for all parameters $\obji \in \objs, \constri \in \constrs$, the objective and constraint functions $\obj[\obji], \constr[\constri]$ are continuous, with the constraint functions additionally satisfying Slater's condition, i.e., $\forall \outer \in \outerset, \exists \inner \in \innerset$ s.t. $\constr[\constri](\outer, \inner) > 0$ for a solution to the optimization problem to exist.

Once again, if in addition one assumes that that the constraint sets $\outerset$ and $\innerset$ are convex, and that for each parameter $\obji \in \objs$, the objective function $\obj[\obji]$ is convex-concave, then $\obj$ is convex-concave and we are guaranteed the existence of a \mydef{generalized saddle point}, i.e., a point $(\outer[][][*], \inner[][][*]) \in \coupledset$ s.t.\ for all $(\outer, \inner[][][*]) \in \coupledset$ and $(\outer[][][*], \inner) \in \coupledset$, $\obj(\outer[][][*], \inner) \leq \obj(\outer[][][*], \inner[][][*]) \leq \obj(\outer, \inner[][][*])$. \amy{need a reference for the guaranteed existence (or a proof in the appendix)}
The relevant game-theoretic model for generalized saddle point problems \amy{not sure, might have to say: stochastic coupled constrained mm opt problems} is the zero-sum pseudo-game,\amy{add reference} a generalization of a zero-sum game with payoffs $\obj$ and $-\obj$ in which the players' actions, not only must lie in individual action sets $\outerset, \innerset$, but are further required to lie in a coupled constraint set $\coupledset$.
The relevant solution concept in pseudo-games is the generalized Nash equilibrium.\amy{add reference} 
In particular, any generalized saddle point can be interpreted as generalized Nash equilibrium, an action profile $(\outer[][][*], \inner[][][*]) \in \coupledset$ at which the players cannot improve their utility by deviating to an action within the set of actions determined their opponent's action, i.e., the sets $\{ \outer \in \outerset \mid (\outer, \inner[][][*]) \in \coupledset\}$ and $\{ \inner \in \innerset \mid (\outer[][][*], \inner) \in \coupledset\}$, respectively.   

Interestingly, while the existence of a Nash equilibrium guarantees that a minimax theorem holds in the uncoupled constraint setting, in the coupled constraint setting, a the existence of a generalized Nash equilibrium does not guarantee that a minimax theorem holds.
In fact, even when the expected objective function $\obj$ is convex-concave, and the coupled constraint set is a polytope, a minimax theorem does not hold in coupled constrained min-max optimization problems \cite{goktas2021minmax}. 
\samy{More importantly}{On the contrary}, the value of a generalized Nash equilibrium is respectively lower and upper bounded by the min-max and max-min optimization problems.
That is, if $(\outer[][][*], \inner[][][*]) \in \coupledset$ is a generalized Nash equilibrium, then 
\begin{align}
    \min_{\outer \in \outerset} \max_{\inner \in \innerset: (\outer, \inner) \in \coupledset} \obj(\outer, \inner) \leq \obj(\outer[][][*], \inner[][][*]) \leq \max_{\inner \in \innerset} \min_{\outer \in \outerset: (\outer, \inner) \in \coupledset} \obj(\outer, \inner)
\end{align}
As a result, coupled constrained min-max optimization problems cannot be interpreted as pseudo-games; nor can their solutions be interpreted as generalized Nash equilibria respectively.
\samy{S}{As suggested by \citet{goktas2021minmax}, s}uch optimization problem are better interpreted as a two-player zero-sum sequential, i.e., \mydef{min-max Stackelberg games},
% \footnote{Throughout this paper, we refer to Stackelberg games with stochastic payoffs as stochastic Stackelberg games, and use the Markov Stackelberg game terminology to refer to repeated Stackelberg games with stochastic transitions \cite{goktas2022zero}.}
where the $\outer$-player, also called the leader, first commits to an action $\outerpoint \in \outerset$, after which the $\inner$-player, also called the follower, having observed the leader's action, makes their own move $\innerpoint(\outerpoint) \in \left\{\inner \in \innerset \mid (\outer, \inner) \in \coupledset \right\}$. 

Define the \mydef{marginal function}%
\footnote{\citet{goktas2021minmax} use the value function terminology to refer to the marginal function but we reserve this terminology for Markov Stackelberg games in this paper.} 
$\val(\outer) \doteq \max_{\inner \in \innerset: (\outer, \inner) \in \coupledset} \obj(\outer, \inner)$.
The solution of any coupled constrained min-max optimization problem---hereafter min-max Stackelberg game---can be interpreted as a Stackelberg equilibrium, a tuple $(\outer[][][*], \inner[][][*]) \in \coupledset$, at which $\outer[][][*] \in \argmin_{\outer \in \outerset} \val(\outer)$ and $\inner \in \argmax_{\inner \in \innerset : (\outer, \inner) \in \coupledset} \obj(\outer, \inner)$.

\citet{goktas2021minmax} identify the class of convex-concave min-max Stackelberg games, i.e., games where $\val$ is convex and $\obj(\outer, \inner)$ is concave in $\inner$ for all $\outer \in \outerset$, as those for which Stackelberg equilibria can be computed in polynomial-time. 
Interestingly, for such problems, simultaneous gradient descent ascent type algorithms fail to converge to Stackelberg equilibria \cite{goktas2022gda}, leading the authors to develop a nested gradient descent ascent-type algorithm: fixing the current action of the $\outer$-player, in an inner loop, their algorithm computes a saddle point of the Lagrangian relaxation of the $\inner$-player's maximization problem; and then using this solution, in an outer loop, the $\outer$-player runs a step of gradient descent on $\val$. 

Unfortunately, \citeauthor{goktas2021minmax}'s algorithm require exact access to the gradient of the game,\amy{of the game? do you mean $\val$?}.
\samy{}{While this requirement can be met in deterministic problems, it is unrealistic in the natural stochastic generalization:}
\amy{i think i might want to introduce the stochastic generalization until now}

\samy{}{As in most stochastic optimization problems (e.g., Markov decision processes), the gradient of the value function cannot always be computed exactly, but often must be estimated from samples instead (e.g., in reinforcement learning).}
For instance, in applications of min-max Stackelberg games to generative adversarial equilibrium solvers to solve economic models \cite{goktas2023generative}, \amy{i don't think you can refer to this paper as an example. at least not right here. because it totally gives away who the authors are. up til now, we are the ONLY authors cited. that may be totally legitimate (if we are pushing new frontiers), but i still don't think the reviewers will like it.} the loss function is a loss which consists of an expectation over a distribution of economic models; this loss and its gradient can only be estimated from samples.
\citeauthor{goktas2021minmax}'s algorithm cannot be used to solve such problems, pointing to the need to develop algorithms that can solve min-max Stackelberg games from noisy estimates of the gradient of the loss \amy{loss? not the marginal/value fn?} functions.

Additionally, such methods can also allow us to develop efficient reinforcement learning for a large class of zero-sum Markov Stackelberg games using variants of policy gradient algorithms, since any Markov Stackelberg game is an instance of a min-max Stackelberg game. Zero-sum Markov Stackelberg games are a generalization for Markov games

}

==> model.tex <==
\section{Min-max Optimization with Fixed Choice Set}

\subsection{Simultaneous Games}

Let $X \subset \mathbb{R}^{n}$ and $Y \subset \mathbb{R}^{m}$ be compact convex sets. Let $f: \R^n \times \R^m \to \R$. Consider the following min-max optimization problem with fixed choice sets:

\begin{align}
    \min_{\x \in  X} \max_{\y \in Y} f(\x, \y)\label{min-max}
\end{align}

One way to see this optimization problem is as a \mydef{simultaneous two-player zero-sum game} where the outer player is trying to minimize their loss and the inner player is trying to maximize their payoff. A two-player zero-sum game is a game of two players with a common payoff function $f: X \times Y \rightarrow \mathbb{R}$. The function $f$ maps the actions taken by both players $(\x, \y) \in X \times Y$ to a real value, which represents the gain of $\y$-player as well as the loss of $\x$-player. We call $\y$ player, who tries to maximize the payoff function $f$, the max-player, and $\x$-player the min-player. In this paper, we focus on continuous payoff functions $f$, and assume $X \subset \mathbb{R}^{d_{1}}$ and $Y \subset \mathbb{R}^{d_{2}}$.

Using this game interpretation, we can then model a solution of this optimization problem as a Nash equilibrium.

\begin{definition}
A tuple $(\x^*,\y^*)$ is called a \mydef{(Global) Nash-equilibrium (NE)} of the game $(n, m, X, Y, f)$ if:
%
\begin{align}
    f(\x^*, \y) \leq f(\x^*, \y^*) \leq f(\x, \y^*) && \forall \x \in X, \y \in Y
\end{align}
\end{definition}

In cases when Nash-equilibria are not unique, we might consider computing \mydef{local Nash equilibria} as we might not reach global Nash equilibria. 

\begin{definition}
A tuple $(\x^*,\y^*)$ is called a \mydef{local Nash-equilibrium (NE)} of the game $(n, m, X, Y, f)$ if there exists a neighborhood $U \subset X \times Y$ of $(\x^*,\y^*)$ such that:
%
\begin{align}
    f(\x^*, \y) \leq f(\x^*, \y^*) \leq f(\x, \y^*) && \forall (\x, \y) \in U
\end{align}
\end{definition}

\begin{proposition}[First-order Necessary Condition]\label{first-order-ness-ne}
Assuming $f$ is differentiable, any local Nash equilibrium satisfies $\nabla_{\mathbf{x}} f(\mathbf{x}, \mathbf{y})=0$ and $\nabla_{\mathbf{y}} f(\mathbf{x}, \mathbf{y})=0$
\end{proposition}

That is, the necessary first order condition for a point to be a Nash equilibirium is that it is a stationary point. 

\begin{proposition}[Second-order Necessary Condition]\label{second-order-ness-ne}
Assuming $f$ is twice-differentiable, any local Nash equilibrium satisfies $\grad[\x \x]^{2} f(\x, \y) \succeq \mathbf{0}$, and $\grad[\y \y]^{2} f(\x, \y) \preceq \mathbf{0}$.
\end{proposition}

The necessary second order condition states that $f$ needs to be locally convex in $\x$ and locally concave in $\y$. From the first and second order necessary conditions, we can see that if the function is convex-concave, then the global Nash equilibrium is a solution that is optimal for \cref{min-max}, since both conditions together imply that the Nash equilibrium is a a global maximum along $\x$ and and a global minimum along $\y$. Similarly, for non-convex-non-concave settings, where multiple saddle-points might exist\footnote{although note that they might not exist at all}, then the local Nash equilibrium is a local maximum along $\x$ and and a local minimum along $\y$.


\begin{proposition}[Second-order Sufficient Condition]
Assuming $f$ is twice-differentiable, any stationary point (i.e., $\nabla f=0$ ) satisfying the following condition is a local Nash equilibrium:

\begin{align}
    \nabla_{\mathbf{y y}}^{2} f(\mathbf{x}, \mathbf{y}) \prec \mathbf{0}, \text { and } \nabla_{\mathbf{x x}}^{2} f(\mathbf{x}, \mathbf{y}) \succ \mathbf{0}  \label{strict-nash-cond}
\end{align}
\end{proposition}
 
We also call a stationary point satisfying \cref{strict-nash-cond} a \mydef{strict local Nash equilibrium}. When $f$ is convex-concave a Nash equilibrium always exists. However, in the non-convex non-concave regime, computing Nash-equilibria is in general NP-Hard. In fact, even finding local Nash equilibria is NP-hard in the general non-convex non-concave regime. One significant drawback of considering local or global Nash equilibria in nonconvex-nonconcave settings is that they may not exist even for simple well-behaved functions.

\begin{theorem}
There exists a twice-differentiable function $f$, where pure strategy Nash equilibria (either local or global) do not exist.
\end{theorem}

\begin{proof}
Consider a two-dimensional function $f(x, y)=\sin (x+y)$. We have $\nabla f(x, y)=(\cos (x+y), \cos (x+$
$y$ )). Assuming $(x, y)$ is a local pure strategy Nash equilibrium, by \cref{first-order-ness-ne} it must also be a stationary point; that is, $x+y=(k+1 / 2) \pi$ for $k \in \mathbb{Z}$. It is easy to verify, for odd $k, \nabla_{x x}^{2} f(x, y)=\nabla_{y y}^{2} f(x, y)=1>0$; for even $k, \nabla_{x x}^{2} f(x, y)=\nabla_{y y}^{2} f(x, y)=-1<0 .$ By \cref{second-order-ness-ne}, none of the stationary points is a local pure strategy Nash equilibrium.
\end{proof}

In such cases, one might consider a relaxed solution concept called the \mydef{the first order Nash-equilibrium} \cite{nouiehed2019solving}. 
%
\begin{definition}
A tuple $(\x^*,\y^*)$ is called a \mydef{first order Nash-equilibrium (FNE)} of the game $(n, m, X, Y, f)$ if:
%
\begin{align}
 \forall \y \in Y,  \langle \grad[\x]f(\x^*, \y^*), \x - \x^* \rangle \geq 0 \text{ and } \forall \x \in X,  \langle \grad[\y]f(\x^*, \y^*), \x - \x^* \rangle \leq 0 
\end{align}
\end{definition}
%
In the absence of constraint sets, $(X, Y)$, the above definition simplifies to $\grad[\x]f(\x^*, \y^*) = 0$ and $\grad[\y]f(\x^*, \y^*) = 0$, which are the well-known unconstrained first-order optimality conditions. The relaxation essentially does not require our solution to be a stationary point, it suffices if the solution is a boundary solution that is a min-max solution, i.e., a minimum along $\x$ and maximum along $\x$ within the feasible region. In the absence of constraints, there exists no boundary solutions and hence, we are back to the regular definition NE.

The following theorem establishes the existence of FNE in setting where the constraint sets are compact and convex:
%
\begin{theorem}
 Suppose the sets $X$ and $Y$ are non-empty, compact, and convex. Moreover, assume that the function $f(\cdot, \cdot)$ is twice continuously differentiable. Then there exists a feasible point $(\x^*, \y^*)$ that is a first-order Nash equilibrium.
\end{theorem}
%
The above theorem guarantees existence of FNE points even when (local) Nash equilibria may not exist. The next natural question is about the computability of such methods. Since in practice we use iterative methods for computation, we need to define the notion of approximate–FNE.

\begin{definition}[Approximate FNE]
A point $\left(\x^{*}, \y^{*}\right)$ is said to be an $\varepsilon$-first-order Nash equilibrium ($\varepsilon$-FNE) of the game $(n, m, X, Y, f)$ if
$$
\mathcal{X}\left(\x^{*}, \y^{*}\right) \leq \varepsilon \quad \text { and } \quad \mathcal{Y}\left(\x^{*}, \y^{*}\right) \leq \varepsilon
$$
where
$$
\mathcal{X}\left(\x^{*}, \y^{*}\right) \triangleq-\min _{\x}\left\langle\nabla_{\x} f\left(\x^{*}, \y^{*}\right), \x-\x^{*}\right\rangle \text { s.t. } \x \in \Theta,\left\|\x-\x^{*}\right\| \leq 1
$$ and $$
\mathcal{Y}\left(\x^{*}, \y^{*}\right) \triangleq \max _{\y}\left\langle\nabla_{\y} f(\x, \y), \y-\y^{*}\right\rangle \text { s.t. } \y \in \mathcal{A},\left\|\y-\y^{*}\right\| \leq 1
$$
\end{definition} 

In the absence of constraints, $\varepsilon$-FNE, reduces to $\left\|\nabla_{\theta} f\left(\x^{*}, \y^{*}\right)\right\| \leq$ $\varepsilon$ and $\left\|\nabla_{\y} f\left(\x^{*}, \y^{*}\right)\right\| \leq \varepsilon$.

\subsection{Sequential Games}
A min-max optimization problems can also be seen as a sequential game. Without loss of generality,  in this paper we assume that the min-player is the first player, and the max-player is second. The objective of this game corresponds to \cref{min-max}. This order does not matter for convex-concave $f(\cdot, \cdot)$, as the minimax theorem guarantees that $\min _{\mathbf{x} \in X} \max _{\mathbf{y} \in Y} f(\mathbf{x}, \mathbf{y})=$ $\max _{\mathbf{y} \in Y} \min _{\mathbf{x} \in X} f(\mathbf{x}, \mathbf{y})$. 

\begin{theorem}{Minimax Theorem}
Let $X \subset \mathbb{R}^{n}$ and $Y \subset \mathbb{R}^{m}$ be compact convex sets. If $f: X \times Y \rightarrow \mathbb{R}$ is a continuous function that is concave-convex, i.e.
$f(\cdot, y): X \rightarrow \mathbb{R}$ is concave for fixed $y,$ and $f(x, \cdot): Y \rightarrow \mathbb{R}$ is convex for fixed $x$
Then we have that
    \begin{align}
        \min _{y \in Y} \max _{x \in X} f(x, y)= \max _{x \in X} \min _{y \in Y} f(x, y)    
    \end{align}
\end{theorem}

For a general nonconvex-nonconcave $f(\cdot, \cdot)$, the minimax theorem does not generally hold and instead we have:
\begin{align}
    \min _{\mathbf{x} \in X} \max _{\mathbf{y} \in Y} f(\mathbf{x}, \mathbf{y}) \neq \max _{\x \in X} \min _{\y \in Y} f(x, y)  
\end{align}
%
This means that the choice of which player goes first plays an important role in the solution. As a result, instead of considering the Nash equilibrium as a solution concept (or in most cases where existence is not guaranteed, the FNE), an alternative solution concept for min-max optimization problems is that of a Stackleberg equilibrium or \mydef{minimax point}\footnote{Minimax point seems to be the term used in the OR community.}. A Stackleberg equilibrium, rather than requiring the outcome to not allow any unilateral utility improving deviations as the Nash equilibrium does, requires the max player to always play a maximizer of $f(\x, \cdot)$ given the action $\x$ taken by the min player (the first player) and achieve the minimum $V(\x) = \max_{\y \in Y} f(\x, \y)$.

\begin{definition}[Minimax Point]
$\left(\mathbf{x}^{\star}, \mathbf{y}^{\star}\right)$ is a global minimax point, if for any $(\mathbf{x}, \mathbf{y})$ in $X \times Y$ we have:
\begin{align}
    f\left(\mathbf{x}^{\star}, \mathbf{y}\right) \leq f\left(\mathbf{x}^{\star}, \mathbf{y}^{\star}\right) \leq \max _{\mathbf{y}^{\prime} \in Y} f\left(\mathbf{x}, \mathbf{y}^{\prime}\right)
\end{align}
\end{definition}
%
\begin{remark}
    Equivalently, $\left(\mathbf{x}^{\star}, \mathbf{y}^{\star}\right)$ is a global minimax point if and only if $\mathbf{y}^{\star}$ is a global maximum of $f\left(\mathbf{x}^{\star}, \cdot\right)$, and $\mathbf{x}^{\star}$ is a global minimum of $\phi(\cdot)$ where $\phi(\mathbf{x}):=\max _{y \in Y} f(\mathbf{x}, \mathbf{y})$.
\end{remark}
%
Unlike Nash equilibria, a global minimax point always exists even if $f$ is nonconvex-nonconcave, due to the extreme-value theorem.
%
\begin{theorem}
    Assume that function $f: X \times Y \rightarrow \mathbb{R}$ is continuous, and assume that $X \subset \mathbb{R}^{n}, Y \subset \mathbb{R}^{m}$ are compact. Then the global minimax point of $f$ always exists.
\end{theorem} 

Finding global minimax points of nonconvex-nonconcave functions is also NP-hard in general. A practical solution is to find a local surrogate. Unfortunately, to the best of our knowledge, there is no formal definition of a local notion of global minimaxity in the literature.


\subsection{Gradient Descent-Ascent Dynamics}

Until very recently there were no first order methods whose last iterate converged to the the solution of the min-max problem even in the concave-convex setting. (Note: there did exist methods whose average iterates converges to the min-max solution). \citeauthor{daskalakis2018limit} consider the issue of no dynamics existing that converge to min-max equilibria and analyze two first order methods/dynamics, the \mydef{gradient descent-ascent (GDA)} dynamics  and the \mydef{optimistic gradient descent-ascent (OGDA)}  dynamics.

The GDA dynamic is defined as:

\begin{align}
    \x^{t+1} = \x^t - \alpha \grad[\x] f(\x^t, \y^t)\\
    \y^{t+1} = \y^t + \alpha \grad[\y] f(\x^t, \y^t)
\end{align}

where $\alpha > 0 $ is the learning rate.

The OGDA dynamic is defined as:

\begin{align}
    \x^{t+1} = \x^t - 2\alpha \grad[\x] f(\x^t, \y^t) + \alpha \grad[\x] f(\x^{t-1}, \y^{t-1})\\
    \y^{t+1} = \y^t + 2\alpha \grad[\y] f(\x^t, \y^t) - \alpha \grad[\y] f(\x^{t-1}, \y^{t-1})
\end{align}

\citeauthor{daskalakis2018limit} show that both dynamics have both stable and unstable fixed points. That is, they prove that not all fixed points of the dynamics are stable. However, this result is not discouraging as the authors prove the following results regarding the convergence of GDA and OGDA:


\begin{theorem} 
Let $\left(\mathbf{x}^{*}, \mathbf{y}^{*}\right)$ be GDA-unstable. Assume $\mu$ is a measure of the starting points $\left(\mathbf{x}_{0}, \mathbf{y}_{0}\right)$ and is absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^{n+m}$. Then it holds that
$$ \operatorname{Pr}\left[\lim _{t}\left(\mathbf{x}_{t}, \mathbf{y}_{t}\right)=\left(\mathbf{x}^{*}, \mathbf{y}^{*}\right)\right]=0 $$
\end{theorem}

\begin{theorem}
Let $\left(\mathbf{x}^{*}, \mathbf{y}^{*}\right)$ be GDA-unstable. Assume $\mu$ is a measure of the starting points $\left(\mathbf{x}_{0}, \mathbf{y}_{0}\right)$ and is absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^{n+m}$. Then it holds that
$$
\operatorname{Pr}\left[\lim _{t}\left(\mathbf{x}_{t}, \mathbf{y}_{t}\right)=\left(\mathbf{x}^{*}, \mathbf{y}^{*}\right)\right]=0
$$
\end{theorem} 

Unfortunately, it turns out that even though GDA and ODGA converge, their stable points are not necessarily min-max solutions, in particular the following relationship holds between min-max saddle points and the stable points of GDA and OGDA:

\begin{align}
    \text{Local Nash-Equilibrium} \subset \text{GDA Stable Point} \subset \text{OGDA Stable Point}
\end{align}

\subsection{A First-Order Method via Danskins' Theorem}

Let $X \subset \mathbb{R}^{n}$ and $Y \subset \mathbb{R}^{m}$ be compact convex sets. Let $f: \R^n \times \R^m \to \R$. Consider the optimization problem $\max_{\y \in Y} f(\x, \y)$ parametrized by $\y \in Y$. The \mydef{value function}, $V: \R^n \to \R$ associated with this maximization problem is defined as:
%
\begin{align}
    V(x) = \max_{\y \in Y} f(\x, \y)\label{value-func}
\end{align}
%
The \mydef{solution correspondence}, $Y^*: \R^n \rightrightarrows \R^m$, associated with $\max_{\y \in Y} f(\x, \y)$ is defined as:
%
\begin{align}
    Y^*(x) = \argmax_{\y \in Y} f(\x, \y)\label{value-func}
\end{align}


Danskin's theorem provides results regarding the convexity and differentiability of the value function:

\begin{theorem}
Suppose that $f: \R^n \times Z \subset \R^m \to \R$ is a continuous function, convex in $\x \in \R^n$ for all $\y \in Y$, with $Z$ compact. Denote the value function and the solution correspondence associated with $\max_{\y \in Y} f(\x, \y)$, by $V: \R^n \to \R$, $Y^*: \R^n \rightrightarrows \R^m$ respectively. Then:
%
\begin{enumerate}\itemsep0em
    \item (Convexity) The value function $V$ is convex
    \item (Derivatives) If $Y$ is singleton-valued, i.e., it is a function, then $V$ is differentiable. Let $\y^*(\x) \in Y^*(\x)$, then $V$ has partial derivatives given by:
    \begin{align}
        \frac{dV(\x)}{dx_i} = \frac{\partial f(\x, \y^*(\x))}{\partial x_i} && \forall i \in [n]
    \end{align}
    \item (Subdifferentials) If $f(\x,\y)$ is differentiable with respect to $\x$ for all $\y \in Y$, and $\frac{\partial f(\x, \y)}{\partial \x}$ is continuous in $\y$ for all $\x$, then the subdifferential of $f$ at a point $\a$ is given by:
    \begin{align}
        \subdiff[\x] V(\x) = \mathrm{conv}\left\{ \frac{\partial f(\x, \y)}{\partial \x} \mid \forall \y \in Y^*(\x)\right\}
    \end{align}
\end{enumerate}
where $\mathrm{conv}$ is the convex hull operation. One can think of this simply as a convex combination of all the derivatives for all solutions given by the solution function.
\end{theorem}

\citeauthor{nouiehed2019solving} propose the following algorithm to solve for $\varepsilon$-FNE:

\begin{center}
    \begin{tabular}{l} 
    Algorithm 1 Multi-step Gradient Descent Ascent \\
    \hline 1: INPUT: $K, T, \eta_{1}=1 / L_{22}, \eta_{2}=1 / L, \y_{0} \in \mathcal{A}$ and $\x_{0} \in \Theta$ \\
    2: for $t=0, \cdots, T-1 \mathbf{do}$ \\
    3: $\quad$ Set $\y_{0}\left(\x_{t}\right)=\y_{t}$ \\
    4: $\quad$ for $k=0, \cdots, K-1 \mathbf{d o}$ \\
    5: $\quad \quad \operatorname{Set} \y_{k+1}\left(\x_{t}\right)=\y_{k}\left(\x_{t}\right)+\eta_{1} \nabla_{\y} f\left(\x_{t}, \y_{k}\left(\x_{t}\right)\right)$ \\
    6: $\quad$ end for \\
    7: $\quad$ Set $\x_{t+1}=\operatorname{proj}_{X}\left(\x_{\mathrm{t}}-\eta_{2} \nabla_{\x} \mathrm{f}\left(\x_{\mathrm{t}}, \y_{\mathrm{K}}\left(\x_{\mathrm{t}}\right)\right)\right)$ \\
    8: end for \\
    9: $\operatorname{Return}\left(\x_{t}, \y_{K}\left(\x_{t}\right)\right)$ for $t=0, \cdots, T-1$
    \end{tabular}
\end{center}

\section{Min-max Optimization with Variable Choice Set}
In the min-max problem given in \cref{min-max}, the choice sets of the players are assumed to be fixed sets. However, in many domain of interest, we are interested in solving min-max optimization problems with variable choice sets. 

Let $X: Y \subset \R^m  \rightrightarrows \R^{n}$ and $Y: : X \subset \R^n  \rightrightarrows \R^{m}$ be compact valued correspondences. Let $f: \R^n \times \R^m \to \R$ be a continuous function. Consider the following min-max optimization problem with variable choice sets:
%
\begin{align}
    \min_{\x \in  X(\y)} \max_{\y \in Y(\x)} f(\x, \y)
\end{align}
%
A solution concept relevant to this min-max optimization problem is that of the minimax point or the Stackleberg equilibrium\footnote{Note that, although \citeauthor{nouiehed2019solving} \cite{nouiehed2019solving} state that they are solving for FNE, however as far as I understand what they are really solving for is the minimax point, which seems to a stronger equilibrium concept.}
Now consider the following value function associated with the inner maximization problem in \cref{min-max-var} :

\begin{align}
    V(\x) = \max_{\y \in Y(\x)} f(\x, \y)\label{value-func-var}
\end{align}
Berge's maximum theorem gives us important conclusion about the value function:
\begin{theorem}[Maximum Theorem]
Consider the class of parametric constrained optimization problems
\begin{align}
    \max _{y \in Y(\x)} f(\x, \y)
\end{align}
defined over the set of parameters $X$. Suppose that (1) $Y: X \rightrightarrows Y$ is continuous (i.e. lsc and usc) and compact-valued, and (2) $f: X \times Y \rightarrow \mathbb{R}$ is a continuous function. Let $Y^{*}(\x) = \argmax _{\y \in Y(\x)} f(\x, \y)$ and, $V(\x) = \max _{\x \in Y(\x)} f(\x, \y)$, then:
\begin{enumerate}
    \item $Y^{*}(\x)$ is non-empty for every $\x \in X$
    \item $Y^{*}$ is upper semi-continuous (and thus continuous if $Y^{*}$ is single-valued)
    \item $V$ is continuous
\end{enumerate}
\end{theorem}
Now going back to our min-max optimization problem \cref{min-max-var}, let $\y^*(\x) \in Y^*(\x)$we can then re-write the min max optimization as:

\begin{align}
    \min_{\x \in X(\y^*(\x))} V(\x)
\end{align}

By Berge's maximum theorem, $V$ is then well-defined and continuous. As a result, we can simply use gradient descent on $V$ to solve this optimization problem. Solving the problem in this way clearly gives us a minimax point:

\begin{align}
    \x^{t+1} = \x^t - \alpha \grad[\x] V(\x^{t-1})
\end{align}

where $\alpha > 0$ is the learning rate.

We know that this gradient descent procedure converges to a local minimum for non-convex functions and to a global minimum for convex functions. The question now boils down to computing $\grad[\x] V(\x^{t-1})$. Lucky for us, economist have discovered the envelope theorem.

\begin{theorem}[Envelope Theorem]
    Consider the maximization problem
    \begin{align}
        \max _{\y \in \R^{n}} f(\x, \y) \text { subject to } g_{k}(\x, \y) \leq b_{k} \text { for all } k=1, \ldots, K    
    \end{align}
    and suppose that (1) $f, g_{1}, \ldots, g_{K}$ are continuous and concave in $\y$, (2) $\partial f / \partial \theta$, $\partial g_{1} / \partial \theta, \ldots, \partial g_{K} / \partial \theta$ are continuous in $(\x, \y)$; and (3) there is some $\widehat{\y} \in \mathbb{R}^{n}$
    such that $g_{k}(\x, \widehat{\y})>0$ for all $k=1, \ldots, K$ and all $\x \in X .$ Then at any point $\hat{\x}$ where $V(\x)$ is differentiable:
    \begin{align}
        \frac{\partial V(\widehat{\x})}{\partial x_{i}}=\frac{\partial f\left( \widehat{\x}, \y^{*}(\widehat{\x})\right)}{\partial x_{i}}-\sum_{k=1}^{K} \lambda_{k} \frac{\partial g_{k}\left(\widehat{\x}, \y^{*}(\widehat{\x})\right)}{\partial x_{i}}
    \end{align}
    where $\lambda_{1}, \ldots, \lambda_{I}$ are the Lagrange multipliers associated associated with $y^{*}(\widehat{\x})$
\end{theorem}


\subsection{Examples}
The dual of the Eisenberg-Gale program which computes equilibrium prices $\price^*$ for any homothetic Fisher $(\util, \budget)$ is given by:

\begin{align}
    \min_{\price \geq 0} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \max_{\allocation[\buyer]: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \util[\buyer](\allocation[\buyer])\right)
\end{align}

Maximizing $\util[\buyer](\allocation[\buyer])$ constrained by the budget of the buyer is equivalent to maximizing $\budget[\buyer] \log \left( \util[\buyer](\allocation[\buyer])\right)$ constrained by the budget of the buyer:

\begin{align}
    \min_{\price \geq 0} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \max_{\allocation[\buyer]: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer])\right)
\end{align}


Notice that we can pull the max outside of the sum because the utility maximization problem for each buyer is independent of the other, giving us:

\begin{align}
    \min_{\price \geq 0} \sum_{\good \in \goods} \price[\good] + \max_{\allocation: \allocation \price \leq \budget} \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer])\right)
\end{align}

Finally, since the variables over which the objective is maximized is independent of the prices, we can pull the maximum entirely our of the expression, giving us:

\begin{align}
    \min_{\price \geq 0} \max_{\allocation: \allocation \price \leq \budget} \sum_{\good \in \goods} \price[\good] +  \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer])\right)
\end{align}

That is, the computation of a Fisher market equilibrium $(\allocation^*, \price^*)$ is a min-max optimization over the sum of the auctioneer's welfare and the Nash social welfare of buyers. Notice, that in the case of the inner optimization problem, the choice set is dependent on the price vector $\price$ selected by the first player, i.e., the auctioneer. As a result, we cannot use first order methods defined that are currently known to solve this problem. However, we can use the envelope theorem and the first order method we just proposed to solve this problem!

\subsection{Proposed Paper Organization}

\begin{enumerate}
     \item Motivating example: Fisher markets
    \item General problem statement: Min-max optimization with variables sets
    \item MAIN TOOL: envelope theorem, solution concepts
    \item Algorithm
    \item Proof of convergence in continuous time (convex-concave + probably non-convex-non-concave)
    \item Convergence in discrete time depends on the $\gamma$-Bregman property (and this property holds in Fisher markets for at least t\^atonnement and proportional response dynamics)  
    \item Future Work: Proof of convergence in discrete time in convex-concave (maybe nonconvex-nonconcave?)
    \item Experiments:
    \begin{itemize}
        \item
        Domains: Simulated simple numeric example; Fisher market equilbria; Fairness example (Future work)
        \item Algorithms:
        \begin{itemize}
        \item Vanilla t\^atonnement (GGD)---inside is closed form for Leontief (a demand oracle)
        \item new t\^atonnement algorithm (gradient descent ascent; GDA)
        \item better baseline: old (2019) algorithm based on Danskins' theorem
        \item proportional response dynamics (?)
        \end{itemize}
        \item Metrics: convergence rates
    \end{itemize}
\end{enumerate}

